Selling Information while Being an Interested Party

We study the algorithmic problem faced by an information holder (seller) who wants to optimally sell such information to a budged-constrained decision maker (buyer) that has to undertake some action. Differently from previous, we consider the case in which the seller is an interested party, as the action chosen by the buyer does not only influence their utility, but also seller's one. This happens in many real-world settings, where the way in which businesses use acquired information may positively or negatively affect the seller, due to the presence of externalities on the information market. The utilities of both the seller and the buyer depend on a random state of nature, which is revealed to the seller, but it is unknown to the buyer. Thus, the seller's goal is to (partially) sell their information about the state of nature to the buyer, so as to concurrently maximize revenue and induce the buyer to take a desirable action. We study settings in which buyer's budget and utilities are determined by a random buyer's type that is unknown to the seller. In such settings, an optimal protocol for the seller must propose to the buyer a menu of information-revelation policies to choose from, with the latter acquiring one of them by paying its corresponding price. Moreover, since in our model the seller is an interested party, an optimal protocol must also prescribe the seller to pay back the buyer contingently on their action. First, we show that the problem of computing a seller-optimal protocol can be solved in polynomial time. Next, we switch the attention to the case in which a seller's protocol employs a single information-revelation policy, rather than proposing a menu, deriving both positive and negative results.

==> content/budget_free.tex <==
\section{Budget Free}
We now switch our attention to the case where the seller has no access to the receiver's type. In particular, in this section, we focus on the simpler case in which the seller may not charge the buyer an initial payment for the selected signaling scheme, $i.e.$, $p=0$.
This setting directly extends the one presented by Dughmi, considering a buyer (receiver) with possibly many types.









==> content/prelim__Copia_in_conflitto_di_Alberto_Marchesi_2023-01-20_.tex <==
\section{Preliminaries}\label{sec:preliminaries}


We study the problem faced by an information holder (\emph{seller}) selling information to a budget-constrained decision maker (\emph{buyer}).
%, who needs to undertake some action.
%
The information available to the seller is collectively termed \emph{state of nature} and encoded as an element of a finite set $\Theta \defeq \{\theta_i\}_{i=1}^d$ of $d$ possible states, while the set of the $m$ actions available to the buyer is $\mathcal{A} \defeq \{a_i\}_{i=1}^m$.
%
The buyer is also characterized by a private \emph{type}, which is unknown to the seller and belongs to a finite set $\mathcal{K} \defeq \{k_i\}_{i=1}^n$ of $n$ possible types.
%
Each buyer's type $k \in \mathcal{K}$ is characterized by a utility function $u^k_\theta:\mathcal{A} \to [0,1]$ associated to each state $\theta \in \Theta$ and a budget $b_k \in \mathbb{R}_{+}$ representing how much they can afford to pay.
%
% Differently from the setting of~\citet{xu2020}, 
%
In our model, the seller's utility is \emph{not} only determined by how much the buyer pays for acquiring information, but it also depends on the buyer's action.
%
Specifically, for every state $\theta \in \Theta$, the sender gets an additional utility contribution determined by a function $u^s_{\theta}:\mathcal{A} \to [0,1]$. 
%
We assume that both the seller and the buyer know the probability distribution $\mu \in \Delta_{\Theta}$ according to which the state of nature is drawn, as well as the probability distribution $\lambda \in \Delta_{\mathcal{K}}$ determining the buyer's type.\footnote{In this work, given a finite set $X$, we let $\Delta_{X}$ be the set of all the probability distributions defined over the elements of $X$.}
%
We let $\mu_\theta$ be the probability assigned to state $\theta \in \Theta$, while $\lambda_k$ is that of type $k \in \mathcal{K}$.


As in~\citep{xu2020}, we assume w.l.o.g. that information revelation happens only once during the seller-buyer interaction.
%
Thus, as it is the case in \emph{Bayesian} persuasion~\citet{kamenica2011bayesian}, the seller reveals information to the buyer by committing to a \emph{signaling scheme} $\phi$, which is a randomized mapping from states of nature to signals being issued to the buyer.
%
Formally, $\phi : \Theta \to \Delta_{\mathcal{S}}$, where $\mathcal{S}$ is a finite set of signals. We denote by $\phi_\theta \in \Delta_{\mathcal{S}}$ the probability distribution employed when the state of nature is $\theta \in \Theta$, with $\phi_\theta(s)$ being the probability of sending $s \in \mathcal{S}$.



An information-selling \emph{protocol} for the seller is defined as follows.
%that the seller implements in order to sell information to the buyer.
%
% In such a protocol,
%
The seller first proposes a \emph{menu} of signaling schemes to the buyer, with each signaling scheme being assigned with a \emph{price}.
%
Then, the buyer chooses a signaling scheme and pays its price upfront, before information is revealed.\footnote{Notice that proposing a menu of signaling schemes is equivalent to asking the buyer to report their type and then choosing a signaling scheme based on that, as it is the case in~\citep{xu2020}.}
%
The seller also commits to action-dependent payments, which are made by the seller in favor of the buyer after information is revealed and the latter has taken an action.
%
This is in contrast with what happens in the protocol introduced by~\citet{xu2020}, where there are no action-dependent money transfers.
%
Intuitively, such payments are needed in order to incentivize the agent to play an action that is profitable for the seller, and, thus, they are \emph{not} needed in the setting of~\cite{xu2020} where the seller's utility function is only determined by how much the buyer pays for acquiring information.
%
Formally, we define a seller's protocol as follows:
%
\begin{definition}[Seller's Protocol]\label{def:protocol}
	A \emph{protocol} for the seller is a tuple $ \{ (\phi^k, p_k,\pi_k ) \}_{k \in \mathcal{K}} $, where:
	\begin{itemize}
		\item $\{\phi^k\}_{k \in \mathcal{K}}$ is a \emph{menu of signaling schemes} $\phi^k: \Theta \to\Delta_{\mathcal{S}}$, one for each receiver's type $k \in \mathcal{K}$; % representing the amount of information the sender discloses to the receiver.
		%
		\item $\{p_k\}_{k \in \mathcal{K}}$ is a \emph{menu of prices}, with $p_k \in \mathbb{R}_+$ representing how much the seller charges the buyer for selecting the signaling scheme $\phi^k$;\footnote{Assuming $p_k \geq 0$ is w.l.o.g., since, intuitively, the seller is never better off paying the buyer before they played any action.}
		%the cost the sender asks to the receiver to sell them the information contained in the signaling scheme $\phi_k$.
		%
		\item $\{\pi_k\}_{k \in \mathcal{K}}$ is a \emph{menu of payment functions}, which are defined as $\pi_k: \mathcal{S} \times \mathcal{A} \to \mathbb{R}_+$ with $\pi_k(s,a)$ encoding how much the seller pays the buyer whenever the latter plays action $a \in \mathcal{A}$ after selecting the signaling scheme $\phi^k$ and receiving signal $s \in \mathcal{S}$.\footnote{The assumption that $\pi_k(s,a) \geq 0$ is w.l.o.g., since the buyer does \emph{not} commit to following the protocol, and, thus, $\pi_k(s,a) < 0$ would result in the buyer leaving the protocol without paying after taking an action.}
	\end{itemize}
\end{definition}
%
%
% Different from the classical Bayesian perusasion framework, we assume that the sender asks the receiver to report their type befoere observing the actual realization of the state of nature. This fact enables the sender to commit to a protocol defined as a menu of signaling schemes and payments. Before describing the actual interaction between the sender and the receiver we report the formal definition of protocol.



The seller and the buyer interact as follows:
%
(i) the seller commits to a protocol $ \{ (\phi^k, p_k,\pi_k  ) \}_{k \in \mathcal{K}} $;
%
(ii) the buyer selects a signaling scheme $\phi^{k}$ and pays $p_{k}$ to the seller (with $k \in \mathcal{K}$ possibly different from their true type);
%
(iii) the seller observes the realized state of nature $\theta \sim \mu$, draws a signal $s \sim \phi^{k}_\theta$ according to the selected signaling scheme, and communicates $s$ to the
buyer; 
%
(iv) given the signal $s$, the buyer infers a posterior distribution $\xi^s \in \Delta_\Theta$ over states of nature, where the probability $\xi^s_\theta$ of state $\theta \in \Theta$ is computed with the \emph{Bayes} rule, as follows:
$$
\xi^s_\theta \defeq \frac{\mu_\theta \, \phi^k_{\theta}(s)}{\sum_{\theta' \in \Theta} \mu_{ \theta'} \phi^k_{\theta'}(s)};
$$
%
(v) given the posterior $\xi^s$, the buyer selects an action $a \in \mathcal{A}$; and
%
(vi) the seller pays $\pi_{k}(s, a)$ to the buyer.
%
As in the model by~\citet{xu2020}, we assume that the seller is committed to following the protocol, while the buyer is \emph{not}, \emph{i.e.}, the buyer is free of leaving the interaction at any point.



In step (v), after observing a signal $s \in \mathcal{S}$ and computing the posterior $\xi^s$, the buyer best responds by choosing an action $a \in \mathcal{A}$ maximizing their expected utility.
%
Formally:
%
\begin{definition}\label{def:br_set}
	Given a signal $s \in \mathcal{S}$, the induced posterior $\xi^s \in \Delta_{\Theta}$, and a payment function $\pi: \mathcal{S} \times \mathcal{A} \to \mathbb{R}_+$, the $\epsilon$-\emph{best-response set} of a buyer of type $k \in \mathcal{K}$ is defined as:
	%
	\[
	\mathcal{B}^k_{\xi^s, \pi} \defeq \argmax_{a\in\mathcal{A}}\sum_{\theta\in\Theta}\xi^s_\theta \, u_\theta^k(a) + \pi(s,a) .
	\]
	We denote by $b_{\xi^s, \pi}^k \in \mathcal{B}^k_{\xi, \pi}$ the best-response action that is actually played by a buyer of type $k \in \mathcal{K}$.\footnote{When the buyer is indifferent among multiple actions, we always assume that they break ties in favor of the seller, choosing the action in $ \mathcal{B}^k_{\xi^s, \pi}$ that maximizes the seller's expected utility.}
\end{definition}
%
\begin{comment}
We also study the case in which the buyer plays an $\epsilon$-best response, meaning that the selected action provides them with an expected utility which is at most $\epsilon$ less than the value of a best response.
%
Formally:
%
\begin{definition}\label{def:eps_br_set}
	Given a signal $s \in \mathcal{S}$, the induced posterior $\xi^s \in \Delta_{\Theta}$, and a payment function $\pi: \mathcal{S} \times \mathcal{A} \to \mathbb{R}_+$, the \emph{$\epsilon$-best-response set} of a buyer of type $k \in \mathcal{K}$ is the set $\mathcal{B}^{\epsilon, k}_{\xi^s, \pi}$ of all the actions $a \in \mathcal{A}$ such that:
	%
	\[
	\sum_{\theta\in\Theta}\p_\theta u_\theta^k(a)+ \pi(s,a) \geq \sum_{\theta\in\Theta}\p_\theta u_\theta^k( a') + \pi(s,a')-\epsilon \quad \forall  a'  \in \mathcal{A}.
	\]
	Moreover, we denote by $b^{\epsilon, k}_{\xi^s, \pi} \in \mathcal{B}^{\epsilon, k}_{\xi^s, \pi}$ the $\epsilon$-best-response action that is actually played by a buyer of type $k \in \mathcal{K}$.\footnote{We assume that, among the actions in the $\epsilon$-best-response set, the buyer always takes the one that is more favorable for the seller.}
\end{definition}
\end{comment}
%
In the following, we will oftentimes work in the space of the posterior distributions $\Delta_{\Theta}$.
%
Thus, given a posterior $\xi \in \Delta_{\Theta}$, we abuse notation and write $\mathcal{B}^k_{\xi, \pi}$ and $b_{\xi, \pi}^k$ by omitting their dependence on a signal $s \in \mathcal{S}$, since this will be clear from context.


The seller's goal is to implement an optimal (\emph{i.e.}, utility-maximizing) protocol $ \{ (\phi^k, p_k,\pi_k ) \}_{k \in \mathcal{K}} $.
%
We focus on seller's protocols that are \emph{incentive compatible} (IC) and \emph{individually rational} (IR).\footnote{By a revelation-principle-style argument (see~\citep{shoham2008multiagent} for some examples), focusing on IC and IR protocols is w.l.o.g. when looking for an optimal protocol.}
%
Specifically, a seller's protocol is IC if for every pair of buyer's types $k, k' \in \mathcal{K}$:
%
\begin{equation*}
\sum_{s \in \mathcal{S}}  \sum_{\theta \in \Theta}  \mu_\theta \phi^k_{\theta}(s) \left[ u^k_\theta(b_{\xi^s, \pi_k}^k) + \pi_k(s,b_{\xi^s, \pi_k}^k) \right] - p_k \ge 
 \sum_{s \in \mathcal{S}} \max_{a \in \mathcal{A}} \sum_{\theta \in \Theta} \mu_\theta \phi^{k'}_{\theta}(s) \left[ u^k_\theta(a) + \pi_{k'}(s, a) \right] - p_{k'} ,
\end{equation*}
%
while it is IR if for every buyers' type $k \in \mathcal{K}$:
%
\begin{equation*}
\sum_{s \in \mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi^k_{\theta}(s) \left[ u^k_\theta(b_{\xi^s, \pi_k}^k) +  \pi_k(s,b_{\xi^s,\pi_k}^k) \right] - p_k \ge 
 \max_{a \in \mathcal{A}}\sum_{\theta \in \Theta} \mu_\theta  u^k_\theta(a) .
\end{equation*}
%
Intuitively, an IC protocol incentivizes the buyer to select the signaling scheme $\phi^{k}$ corresponding ot their true type $k \in \mathcal{K}$, while an IR protocol ensures that the buyer gets more utility by acquiring information rather than leaving the protocol before step (ii) and playing an action without information.
%
Then, the seller's expected utility is computed as follows:
\[
\sum_{k \in \mathcal{K}} \lambda_k \left[ \sum_{s \in\mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi^{k}_\theta(s) \left[ u_\theta^s(b^k_{\xi^s,\pi_k}) -\pi_k(s, b^k_{\xi^s,\pi_k}) \right]+ p_k  \right].
\]

A crucial component of our results is that we can restrict the attention to protocols that are \emph{direct} and \emph{persuasive}.
%
We say that protocol is {direct} if it uses signaling schemes whose signals correspond to action recommendations for the buyer, namely $\mathcal{S} = \mathcal{A}$, while a direct protocol is said to be {persuasive} whenever playing the recommended action is always a best response for the buyer. 
%
%\mat{magari dire che lo dimostriamo dopo? cosi sembra che è ovvio.}


\subsection{Protocols without Menus}

We switch the attention to the case in which the seller does \emph{not} let the buyer selecting form a menu, but they rather commit to a single signaling scheme and a single payment function.\footnote{From the point of view of~\citet{xu2020} , this is equivalent to assuming that there is no type reporting stage.}
%
Analogously to the case with selection, a Seller's Protocol without selection is defined by a tuple $(\phi,p,\pi)$, where $\phi: \Theta \to\Delta_{\mathcal{S}}$ is the signaling scheme, encoding how the seller spreads the information to the buyer, $p \in \mathbb{R}_+$ is the price that the seller initially charges the buyer to reveal them the information, while $\pi: \mathcal{S} \times \mathcal{A} \to \mathbb{R}_+$ is the payment function, describing how much the seller pays the buyer after receiving the information.
%
The seller-buyer interaction unfolds as in the previous case, with step (ii) only involving the payment of a single $p \in \mathbb{R}_+$ which is common among all the buyer's types.
%
It is important to remark that, to take part in the protocol, the buyer is only required to satisfy the IR constraints since the IC constraints are \emph{not} needed without a menu.
%
This model generalizes the one presented in~\citet{dughmi2019} by adding an initial payment from the buyer to the seller.
%
In the following, it will be useful to directly work in the space of distributions over posteriors.
%
In particular, a signaling scheme $\phi: \Theta \to \Delta_{\mathcal{S}}$ induces a distribution $\gamma$ over $\Delta_{\Theta}$ such that $\text{supp}(\gamma) \defeq \left\{ \xi^s \mid s \in \mathcal{S}  \right\}$ and satisfies the following relation:
%
\begin{equation}
\label{eq:consistent}
\sum_{\xi \in \text{supp}(\gamma)} \gamma_\xi \xi_\theta = \mu_\theta \,\,\, \forall \theta \in \Theta
\end{equation}
%
Thus, instead of working with signaling schemes $\phi$, one can w.l.o.g. focus on distributions $\gamma$ over $\Delta_{\Theta}$ that are \emph{consistent} with the prior according to Equation~\eqref{eq:consistent}. It is worth noting that the seller may design a protocol in which only a subset of buyer types may actually participate in the mechanism and consequently buy the information. Specifically, the seller has to determine a subset $ \mathcal{IR} \subseteq \mathcal{K} $ such that each buyer's type $k \in \mathcal{IR}$ (i) have enough budget to buy the information, \emph{i.e.}, $b_k \ge p $; (ii) satisfy the IR constraints, according to the following equation:
\mat{chiamiamo gli IR $\R$ (decidere se mettere a pedice il protocollo).}
%
\begin{equation*}
\sum_{s \in \mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi_{\theta}(s) \left[ u^k_\theta(b_{\xi^s, \pi}^k) +  \pi(s,b_{\xi^s,\pi}^k) \right] - p \ge \sum_{\theta \in \Theta} \mu_\theta  u^k_\theta(a) 
%
\end{equation*}
for each action $a \in \mathcal{A}$. Finally, given a protocol $(\phi, \pi, p)$, the seller's expected utility is given by: 
%
\begin{equation*}
\sum_{k \in \mathcal{IR}} \left[ \lambda_k \sum_{s \in\mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi_\theta(s) \left[ u_\theta^s(b^k_{\xi^s,\pi}) -\pi(s, b^k_{\xi^s,\pi}) \right] + p  \right] + \sum_{k \not \in \mathcal{IR} }\lambda_k \sum_{\theta \in \Theta} \mu_\theta  u^k_\theta(b^k_\mu)
\end{equation*}
where we denote with $b^k_{\mu} \in \arg \max_{a \in \mathcal{A}} \sum_{\theta \in \Theta} \mu_\theta  u^k_\theta(a)$. \mat{, where as customary the receiver breaks ties in favour of the seller.}

\begin{comment}
\begin{subequations}
	\begin{align*}
	& \max_{A \subseteq \mathcal{P}(\K)}\max_{\gamma, p, \pi \ge 0}
	\sum_{k \in A} \lambda_k \sum_{s \in\mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi_\theta(s) \left[ u_\theta^s(b^k_{\xi^s,\pi}) -\pi(s, b^k_{\xi^s,\pi}) \right] \\
	& + p \sum_{k \in A } \lambda_k + \sum_{k \not \in A }\lambda_k \sum_{\theta \in \Theta} \mu_\theta  u^k_\theta(b^k_\mu) \\ 
	&\sum_{s \in \mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi_{\theta}(s) \left[ u^k_\theta(b_{\xi^s, \pi}^k) +  \pi(s,b_{\xi^s,\pi}^k) \right] - p \ge \\
	& \quad \max_{a \in \mathcal{A}}\sum_{\theta \in \Theta} \mu_\theta  u^k_\theta(a) \,\,\,  \forall k \in A \\
	& \sum_{s \in \mathcal{S}} \sum_{\theta \in \Theta} \mu_\theta \phi_{\theta}(s) \left[ u^k_\theta(b_{\xi^s, \pi}^k) +  \pi(s,b_{\xi^s,\pi}^k) \right] - p \le \\
	& \sum_{s \in \mathcal{S}} \mu_\theta  u^k_\theta(b^k_\mu) \,\,\,  \forall k \not \in A \\
	& \sum_{s \in \mathcal{S}} \phi_\theta(s)  = 1  \,\,\,  \forall \theta \in \Theta \\
	& p \le b_k \forall k \in A
	\end{align*}
\end{subequations}
\end{comment}
\subsection{Illustrative Example}

\mat{questa sezione non mi convince per niente.}

We conclude with an illustrative example of the interaction between the seller and  and buyer. Moreover, the example shows that the final signal-action-dependent payment step that we introduce in our protocol enables the seller to obtain utility higher than that achievable without it (\emph{e.g.}, by using the protocol of~\citet{xu2020}, where the seller cannot pay the buyer for their action).

\mat{questo esempio non ha molto senso secondo me. Dovrebbe anche mostrare un po come funziona l'interazione tra i giocatori secondo me}
\begin{example}
	Consider an instance with two states of nature $\Theta \defeq \{\theta_1, \theta_2\}$, a uniform prior distribution, and two buyer's actions $\mathcal{A} \defeq \left\{ a_1,a_2
	\right\}$.
	%
	Moreover, let $u^s_{\theta_1}(a_2)=u^s_{\theta_2}(a_2)=1$ and $u^s_{\theta_1}(a_1)=u^s_{\theta_2}(a_1)=0$. 
	%
	Consider a buyer with limited liability characterized by two types $ k_1, k_2$, such that $\lambda_{k_1}=\lambda_{k_2}=0.5$ with $u^{k_1}_{\theta_1}(a_2)=u^{k_1}_{\theta_2}(a_2)=0$ and $u^{k_1}_{\theta_1}(a_1)=u^{k_1}_{\theta_2}(a_1)=0.5$, while $u^{k_2}_{\theta_1}(a_2)=u^{k_2}_{\theta_2}(a_2)=0$ and $u^{k_2}_{\theta_1}(a_1)=u^{k_2}_{\theta_2}(a_1)=1$.
	%
	In this case we assume that the seller commits to protocol characterized by signaling schemes revealing the buyer the actual state of nature, so that $\mathcal{S}\coloneqq\{s_{\theta_1}, s_{\theta_2}\}$ where $s_\theta$ is the signal revealing th buyer the state $\theta \in \Theta$. Moreover, we assume that the payment functions implemented by the seller are given by $\pi_{k_1}(s,a_1)=0$ and $\pi_{k_1}(s,a_2)= 0.5$, while $\pi_{k_2}(s,a)= 0$ for each $s \in \mathcal{S}$ and action $a \in \mathcal{A}$. It is easy to check the protocol implemented by the seller is IC and IR, since the buyer is not incentivated to misreport their true type. If we assume that the true type of the buyer is $k_1$ we have that, once they report their true type to the seller, if they play action $a_1$ they receive a 
	%
	If the seller cannot pay the buyer after they take an action, then the buyer will play $a_1$ for any signaling scheme $\phi^{k_1}$ proposed by seller, since the buyer gets $0.5$ by playing $a_1$ and $0$ by playing $a_2$, no matter the state of nature.
	%
	As a result the seller's expected utility is $0$.
	%
	Instead, if the seller implements a protocol with $\pi_{k_1}(s,a_2)= 0.5$ and $\pi_{k_1}(s,a_1)=0$ for all $s \in \mathcal{S}$, then the buyer will always play $a_1$ (being indifferent between the two actions), resulting in a seller's expected utility of $0.5$.
\end{example}

\mat{old version}
%
We conclude with an illustrative example showing that the final signal-action-dependent payment step in our protocol enables the seller to obtain utility higher than that achievable without it (\emph{e.g.}, by using the protocol of~\citet{xu2020}, where the seller cannot pay the buyer for their action).
%
% \begin{example}
Consider an instance with two states of nature $\Theta \defeq \{\theta_1, \theta_2\}$, a uniform prior distribution, and two buyer's actions $\mathcal{A} \defeq \left\{ a_1,a_2
\right\}$.
%
Moreover, let $u^s_{\theta_1}(a_2)=u^s_{\theta_2}(a_2)=1$ and $u^s_{\theta_1}(a_1)=u^s_{\theta_2}(a_1)=0$. 
%
Consider a buyer characterized by a single type $ k_1$, with $b_{k_1}= 0$, $u^{k_1}_{\theta_1}(a_2)=u^{k_1}_{\theta_2}(a_2)=0$ and $u^{k_1}_{\theta_1}(a_1)=u^{k_1}_{\theta_2}(a_1)=0.5$.
%
If the seller cannot pay the buyer after they take an action, then the buyer will play $a_1$ for any signaling scheme $\phi^{k_1}$ proposed by seller, since the buyer gets $0.5$ by playing $a_1$ and $0$ by playing $a_2$, no matter the state of nature.
%
As a result the seller's expected utility is $0$.
%
Instead, if the seller implements a protocol with $\pi_{k_1}(s,a_2)= 0.5$ and $\pi_{k_1}(s,a_1)=0$ for all $s \in \mathcal{S}$, then the buyer will always play $a_1$ (being indifferent between the two actions), resulting in a seller's expected utility of $0.5$.
%
% \end{example}










